Asphaltene precipitation under controlled mixing conditions in a microchamber

Solvent exchange is a controlled process for dilution-induced phase separation. This work utilizes the solvent exchange method to reveal the effect of the mixing dynamics on the asphaltene precipitation process under 20 different mixing conditions using a model system of n-heptane and asphaltene in toluene. The external mixing between the asphaltene solution and the paraffinic solvent is strictly controlled. We employed a high-spatial-resolution total internal reflection fluorescence microscope to detect asphaltene precipitates with a resolution up to 200 nm. A multiphysics model is used to simulate the evolution of the oversaturation pulse in the solvent exchange process. Based on the simulation results, we predicted the effect of the flow rate, dimension, the orientation of the microfluidic chamber, and temperature on the surface coverage and size distribution of asphaltene precipitates. The model predictions of all factors corroborate with the experimental observations. Local concentration of the solvent and shear forces are found to be the two main reasons for the change of asphaltene precipitation caused by mixing dynamics. However, the influence of thermodynamics is more critical than the mixing dynamics as temperature changes. Through a combination of experimental and simulation studies, this work illuminates the significance of the transportation process for the final morphology of asphaltene precipitates and provides an in-depth insight into the mechanism of mixing dynamics on the asphaltene precipitation. A smart mixing may be to boost new phase formation without excessive solvent consumption.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
